A GALEX Ultraviolet Imaging Survey of Galaxies in the Local Volume

We present results from a GALEX ultraviolet (UV) survey of a complete sample of 390 galaxies within ~11 Mpc of the Milky Way. The UV data are a key component of the composite Local Volume Legacy (LVL), an ultraviolet-to-infrared imaging program designed to provide an inventory of dust and star formation in nearby spiral and irregular galaxies. The ensemble dataset is an especially valuable resource for studying star formation in dwarf galaxies, which comprise over 80% of the sample. We describe the GALEX survey programs which obtained the data and provide a catalog of far-UV (~1500 Angstroms) and near-UV (~2200 Angstroms) integrated photometry. General UV properties of the sample are briefly discussed. We compute two measures of the global star formation efficiency, the SFR per unit HI gas mass and the SFR per unit stellar mass, to illustrate the significant differences that can arise in our understanding of dwarf galaxies when the FUV is used to measure the SFR instead of H-alpha. We find that dwarf galaxies may not be as drastically inefficient in coverting gas into stars as suggested by prior H-alpha studies. In this context, we also examine the UV properties of late-type dwarf galaxies that appear to be devoid of star formation because they were not detected in previous H-alpha narrowband observations. Nearly all such galaxies in our sample are detected in the FUV, and have FUV SFRs that fall below the limit where the H-alpha flux is robust to Poisson fluctuations in the formation of massive stars. The UV colors and star formation efficiencies of H-alpha-undetected, UV-bright dwarf irregulars appear to be relatively unremarkable with respect to those exhibited by the general population of star-forming galaxies.

==> references.tex <==
\bibitem[Adelman-McCarthy et al.(2006)]{2006ApJS..162...38A} 
Adelman-McCarthy, J.~K., et al.\ 2006, \apjs, 162, 38 
\bibitem[Bigiel et al.(2008)]{2008AJ....136.2846B} Bigiel, F., Leroy, A., 
Walter, F., Brinks, E., de Blok, W.~J.~G., Madore, B., 
\& Thornley, M.~D.\ 2008, \aj, 136, 2846 
\bibitem[Blanton et al.(2005)]{2005ApJ...631..208B} Blanton, M.~R., Lupton, 
R.~H., Schlegel, D.~J., Strauss, M.~A., Brinkmann, J., Fukugita, M., 
\& Loveday, J.\ 2005, \apj, 631, 208
\bibitem[Bothwell et al.(2009)]{2009MNRAS.400..154B} Bothwell, M.~S., 
Kennicutt, R.~C., \& Lee, J.~C.\ 2009, \mnras, 400, 154  
\bibitem[Boselli et al.(2009)]{2009ApJ...706.1527B} Boselli, A., Boissier, 
S., Cortese, L., Buat, V., Hughes, T.~M., 
\& Gavazzi, G.\ 2009, \apj, 706, 1527
\bibitem[Brinchmann et al.(2004)]{2004MNRAS.351.1151B} Brinchmann, J., 
Charlot, S., White, S.~D.~M., Tremonti, C., Kauffmann, G., Heckman, T., 
\& Brinkmann, J.\ 2004, \mnras, 351, 1151 
\bibitem[Cair{\'o}s et al.(2001)]{2001ApJS..133..321C} Cair{\'o}s, L.~M., 
V{\'{\i}}lchez, J.~M., Gonz{\'a}lez P{\'e}rez, J.~N., Iglesias-P{\'a}ramo, 
J., \& Caon, N.\ 2001, \apjs, 133, 321
\bibitem[Cardelli et al.(1989)]{1989ApJ...345..245C} Cardelli, J.~A., 
Clayton, G.~C., \& Mathis, J.~S.\ 1989, \apj, 345, 245 
\bibitem[C{\^o}t{\'e} et al.(2009)]{2009AJ....138.1037C} C{\^o}t{\'e}, S., 
Draginda, A., Skillman, E.~D., \& Miller, B.~W.\ 2009, \aj, 138, 1037  
\bibitem[de Jong et al.(2008)]{2008ApJ...680.1112D} de Jong, J.~T.~A., et 
al.\ 2008, \apj, 680, 1112 
\bibitem[de Vaucouleurs et al.(1991)]{1991trcb.book.....D} de Vaucouleurs, 
G., de Vaucouleurs, A., Corwin, H.~G., Jr., Buta, R.~J., Paturel, G., 
\& Fouque, P.\ 1991, Volume 1-3, XII, 2069 pp.~7 figs..~ Springer-Verlag Berlin Heidelberg New York,  
\bibitem[Dalcanton et al.(2009)]{2009ApJS..183...67D} Dalcanton, J.~J., et 
al.\ 2009, \apjs, 183, 67 
\bibitem[Dale et al.(2009)]{2009ApJ...703..517D} Dale, D.~A., et al.\ 2009, 
\apj, 703, 517
\bibitem[Eldridge(2010)]{2010arXiv1008.1352E} Eldridge, J.~J 2010, 
arXiv:1008.1352  
\bibitem[Fumagalli et al.(2010)]{2010arXiv1009.0524F} Fumagalli, M., da 
Silva, R., Krumholz, M., \& Bigiel, F.\ 2010, arXiv:1009.0524 
\bibitem[Gallagher \& Hunter(1984)]{1984ARA&A..22...37G} Gallagher, J.~S., III, \& Hunter, D.~A.\ 1984, \araa, 22, 37 
\bibitem[Gil de Paz et al.(2003)]{2003ApJS..147...29G} Gil de Paz, A., 
Madore, B.~F., \& Pevunova, O.\ 2003, \apjs, 147, 29 
\bibitem[Gil de Paz et al.(2005)]{2005ApJ...627L..29G} Gil de Paz, A., et 
al.\ 2005, \apjl, 627, L29 
\bibitem[Gil de Paz \& Madore(2005)]{2005ApJS..156..345G} Gil de Paz, A., \& Madore, B.~F.\ 2005, \apjs, 156, 345 
\bibitem[Gil de Paz et al.(2007)]{2007ApJS..173..185G} Gil de Paz, A., et 
al.\ 2007, \apjs, 173, 185 
\bibitem[Goddard et al.(2010)]{2010MNRAS.405.2791G} Goddard, Q.~E., 
Kennicutt, R.~C., \& Ryan-Weber, E.~V.\ 2010, \mnras, 405, 2791
\bibitem[Grebel et al.(2003)]{2003AJ....125.1926G} Grebel, E.~K., 
Gallagher, J.~S., III, \& Harbeck, D.\ 2003, \aj, 125, 1926 
\bibitem[Hodge(1974)]{1974PASP...86..845H} Hodge, P.~W.\ 1974, \pasp, 86, 
845
\bibitem[Hunter 
\& Gallagher(1985)]{1985ApJS...58..533H} Hunter, D.~A., \& Gallagher, J.~S., III 1985, \apjs, 58, 533 
\bibitem[Hunter \& Elmegreen(2004)]{2004AJ....128.2170H} Hunter, D.~A., \& Elmegreen, B.~G.\ 2004, \aj, 128, 2170 
 \bibitem[Hunter et al.(2010)]{2010AJ....139..447H} Hunter, D.~A., 
Elmegreen, B.~G., \& Ludka, B.~C.\ 2010, \aj, 139, 447
\bibitem[James et al.(2008)]{2008A&A...484..703J} James, P.~A., Prescott, M., \& Baldry, I.~K.\ 2008, \aap, 484, 703 
\bibitem[Karachentsev 
\& Makarov(1996)]{1996AJ....111..794K} Karachentsev, I.~D., \& Makarov, D.~A.\ 1996, \aj, 111, 794 
\bibitem[Karachentsev et al.(2004)]{2004AJ....127.2031K} Karachentsev, 
I.~D., Karachentseva, V.~E., Huchtmeier, W.~K., \& Makarov, D.~I.\ 2004, \aj, 127, 2031 
\bibitem[Karachentsev \& Kaisin(2007)]{2007AJ....133.1883K} Karachentsev, I.~D., \& Kaisin, S.~S.\ 2007, \aj, 133, 1883 
\bibitem[Kennicutt(1983)]{1983ApJ...272...54K} Kennicutt, R.~C., Jr.\ 1983, 
\apj, 272, 54 
\bibitem[Kennicutt(1989)]{1989ApJ...344..685K} Kennicutt, R.~C., Jr.\ 1989, 
\apj, 344, 685
\bibitem[Kennicutt(1998a)]{1998ApJ...498..541K} Kennicutt, R.~C., Jr.\ 1998, 
\apj, 498, 541  
\bibitem[Kennicutt(1998b)]{1998ARA&A..36..189K} Kennicutt, R.~C., Jr.\ 1998, \araa, 36, 189 
\bibitem[Kennicutt et al.(1994)]{1994ApJ...435...22K} Kennicutt, R.~C., 
Jr., Tamblyn, P., \& Congdon, C.~E.\ 1994, \apj, 435, 22 
\bibitem[Kennicutt et al.(2008)]{2008ApJS..178..247K} Kennicutt, R.~C., 
Jr., Lee, J.~C., Funes, S.~J., Jos{\'e} G., Sakai, S., 
\& Akiyama, S.\ 2008, \apjs, 178, 247 (Paper I)
\bibitem[Knapen \& James(2009)]{2009ApJ...698.1437K} Knapen, J.~H., \& James, P.~A.\ 2009, \apj, 698, 1437 
\bibitem[Kroupa \& Weidner(2003)]{2003ApJ...598.1076K} Kroupa, P., \& Weidner, C.\ 2003, \apj, 598, 1076 
\bibitem[Lee et al.(2004)]{2004ApJ...616..752L} Lee, J.~C., Salzer, J.~J., 
\& Melbourne, J.\ 2004, \apj, 616, 752 
\bibitem[Lee et al.(2007)]{2007ApJ...671L.113L} Lee, J.~C., Kennicutt, 
R.~C., Funes, S.~J., Jos{\'e} G., Sakai, S., 
\& Akiyama, S.\ 2007, \apjl, 671, L113 
\bibitem[Lee et al.(2009a)]{2009ApJ...692.1305L} Lee, J.~C., Kennicutt, 
R.~C., Jos{\'e} G.~Funes, S.~J., Sakai, S., 
\& Akiyama, S.\ 2009, \apj, 692, 1305 
\bibitem[Lee et al.(2009b)]{2009ApJ...706..599L} Lee, J.~C., et al.\ 2009, 
\apj, 706, 599
\bibitem[Martin et al.(2005)]{2005ApJ...619L...1M} Martin, D.~C., et al.\ 
2005, \apjl, 619, L1 
\bibitem[Mateo(1998)]{1998ARA&A..36..435M} Mateo, M.~L.\ 1998, \araa, 36, 435 
\bibitem[Melena et al.(2009)]{2009AJ....138.1203M} Melena, N.~W., 
Elmegreen, B.~G., Hunter, D.~A., \& Zernow, L.\ 2009, \aj, 138, 1203
\bibitem[Meyer et al.(2004)]{2004MNRAS.350.1195M} Meyer, M.~J., et al.\ 
2004, \mnras, 350, 1195  
\bibitem[Meurer et al.(2009)]{2009ApJ...695..765M} Meurer, G.~R., et al.\ 
2009, \apj, 695, 765
\bibitem[Meurer(2010)]{2010arXiv1008.3946M} Meurer, G.~R.\ 2010, 
arXiv:1008.3946
\bibitem[Miller et al.(2001)]{2001ApJ...562..713M} Miller, B.~W., Dolphin, 
A.~E., Lee, M.~G., Kim, S.~C., \& Hodge, P.\ 2001, \apj, 562, 713   
\bibitem[Morrissey et al.(2005)]{2005ApJ...619L...7M} Morrissey, P., et 
al.\ 2005, \apjl, 619, L7 
\bibitem[Morrissey(2006)]{2006SPIE.6266E..26M} Morrissey, P.\ 2006, 
\procspie, 6266,  
\bibitem[Morrissey et al.(2007)]{2007ApJS..173..682M} Morrissey, P., et 
al.\ 2007, \apjs, 173, 682 
\bibitem[Paturel et al.(2003)]{2003A&A...412...57P} Paturel, G., Theureau, G., Bottinelli, L., Gouguenheim, L., Coudreau-Durand, N., Hallet, N., \& Petit, C.\ 2003, \aap, 412, 57 
\bibitem[Pflamm-Altenburg 
\& Kroupa(2009)]{2009ApJ...706..516P} Pflamm-Altenburg, J., \& Kroupa, P.\ 2009, \apj, 706, 516 
\bibitem[Popescu 
\& Hanson(2010)]{2010arXiv1007.3718P} Popescu, B., \& Hanson, M.~M.\ 2010, arXiv:1007.3718 
\bibitem[Schiminovich et al.(2007)]{2007ApJS..173..315S} Schiminovich, D., 
et al.\ 2007, \apjs, 173, 315 
\bibitem[Schlegel et al.(1998)]{1998ApJ...500..525S} Schlegel, D.~J., 
Finkbeiner, D.~P., \& Davis, M.\ 1998, \apj, 500, 525
\bibitem[Schmidt(1959)]{1959ApJ...129..243S} Schmidt, M.\ 1959, \apj, 129, 
243 
\bibitem[Skillman et al.(1989)]{1989ApJ...347..875S} Skillman, E.~D., 
Kennicutt, R.~C., \& Hodge, P.~W.\ 1989, \apj, 347, 875 
\bibitem[Skillman et al.(2003)]{2003AJ....125..593S} Skillman, E.~D., 
C{\^o}t{\'e}, S., \& Miller, B.~W.\ 2003, \aj, 125, 593 
\bibitem[Springob et al.(2005)]{2005ApJS..160..149S} Springob, C.~M., 
Haynes, M.~P., Giovanelli, R., \& Kent, B.~R.\ 2005, \apjs, 160, 149 
\bibitem[Thilker et al.(2005)]{2005ApJ...619L..79T} Thilker, D.~A., et al.\ 
2005, \apjl, 619, L79 
\bibitem[Thilker et al.(2007)]{2007ApJS..173..538T} Thilker, D.~A., et al.\ 
2007, \apjs, 173, 538 
\bibitem[Tolstoy et 
al.(2009)]{2009ARA&A..47..371T} Tolstoy, E., Hill, V., \& Tosi, M.\ 2009, \araa, 47, 371 
\bibitem[Tremonti et al.(2007)]{2007AAS...211.9503T} Tremonti, C.~A., Lee, 
J.~C., van Zee, L., Kennicutt, R.~C., Gil de Paz, A., Sakai, S., Funes, J., 
\& Akiyama, S.\ 2007, Bulletin of the American Astronomical Society, 38, 894 
\bibitem[Tully(1988)]{1988AJ.....96...73T} Tully, R.~B.\ 1988, \aj, 96, 73 
\bibitem[Tully et al.(2006)]{2006AJ....132..729T} Tully, R.~B., et al.\ 
2006, \aj, 132, 729 
\bibitem[van Zee et al.(1997)]{1997AJ....114.2479V} van Zee, L., Haynes, 
M.~P., \& Salzer, J.~J.\ 1997, \aj, 114, 2479 
\bibitem[van Zee(2001)]{2001AJ....121.2003V} van Zee, L.\ 2001, \aj, 121, 
2003
\bibitem[Weidner 
\& Kroupa(2005)]{2005ApJ...625..754W} Weidner, C., \& Kroupa, P.\ 2005, \apj, 625, 754 
\bibitem[Weidner 
\& Kroupa(2006)]{2006MNRAS.365.1333W} Weidner, C., \& Kroupa, P.\ 2006, \mnras, 365, 1333 
\bibitem[Weisz et al.(2008)]{2008ApJ...689..160W} Weisz, D.~R., Skillman, 
E.~D., Cannon, J.~M., Dolphin, A.~E., Kennicutt, R.~C., Jr., Lee, J., 
\& Walter, F.\ 2008, \apj, 689, 160 
\bibitem[Zaritsky 
\& Christlein(2007)]{2007AJ....134..135Z} Zaritsky, D., \& Christlein, D.\ 2007, \aj, 134, 135 

